Characterizing SARS-CoV-2 Spike Sequences Based on Geographical Location

With the rapid spread of COVID-19 worldwide, viral genomic data is available in the order of millions of sequences on public databases such as GISAID. This Big Data creates a unique opportunity for analysis towards the research of effective vaccine development for current pandemics, and avoiding or mitigating future pandemics. One piece of information that comes with every such viral sequence is the geographical location where it was collected -- the patterns found between viral variants and geographical location surely being an important part of this analysis. One major challenge that researchers face is processing such huge, highly dimensional data to obtain useful insights as quickly as possible. Most of the existing methods face scalability issues when dealing with the magnitude of such data. In this paper, we propose an approach that first computes a numerical representation of the spike protein sequence of SARS-CoV-2 using $k$-mers (substrings) and then uses several machine learning models to classify the sequences based on geographical location. We show that our proposed model significantly outperforms the baselines. We also show the importance of different amino acids in the spike sequences by computing the information gain corresponding to the true class labels.

==> Makefile <==
targets = \
	main.pdf abstract.txt \
	main-csl-trunc.pdf latex_sources.zip
subdirs =

all : $(targets) subdirs

%.pdf : %.tex references.bib cslsec.tex
	latexmk -pdf $< && latexmk -c $<

%-trunc.pdf : %.pdf
	pdftk $< cat 1-29 output $@

%-csl.tex : %.tex
	sed 's/^\\bibliographystyle.*/\\input{cslsec.tex}\n&/' $< > $@

abstract.txt : main.tex
	grep -A 1000 "begin{abstract}" $< | tail -n +2 \
		| grep -B 1000 "end{abstract}" | head -n -1 \
		| sed '/begin{comment}/, /end{comment}/ s|^|%|' \
		| sed 's/^\\textcolor.*/%&/' \
		| sed 's/^%.*//' > $@

# for latex sources
#----------------------------------------------------------------------
%.zip : %
	zip -r $@ $<
	rm -rf $<

template_files = Liebert_Author.cls mary-ann-liebert-harvard.csl
figures_dirs = Figures Tikz_Figures
latex_sources : main.tex references.bib
	rm -rf $@
	mkdir -p $@
	cp $^ $(template_files) $@
	cp -r $(figures_dirs) $@

# kludge for JCB bibliographic format based on provided csl
#----------------------------------------------------------------------
cslsec.tex : cslbib.tex
	echo "\section*{References}" > $@
	echo "\\\vspace*{-.5cm}" >> $@
	cat $< >> $@
	echo "\\\clearpage" >> $@

cslbib.tex : pandoc.tex
	grep -A 1000 "\hypertarget{refs}{}" $< | \
	sed 's/\\leavevmode/\\vspace*{.5cm}\n\\noindent%/' > $@

pandoc.tex : citations.tex references.bib mary-ann-liebert-harvard.csl
	pandoc $< \
		--bibliography=references.bib \
		--csl=mary-ann-liebert-harvard.csl \
		-o $@

citations.tex : main.tex
	egrep -o "\\\cite{[^}]*}" $< > $@

# for building in the subdirectories (figures, etc.)
#----------------------------------------------------------------------
.PHONY : subdirs
subdirs : $(subdirs)
	for subdir in $^ ; do \
		cd $$subdir && make && cd .. ; \
	done

# cleanup
.PHONY : clean scour
clean :
	rm -f *~
	rm -f *.aux *.bbl *.log *.out
	rm -f *.fdb_latexmk *.fls *.auxlock
	rm -f citations.tex pandoc.tex cslbib.tex cslsec.tex
	rm -f main-csl.tex main-csl.pdf

scour : clean
	rm -rf $(targets)

